Fair, Manipulation-Robust, and Transparent Sortition

Sortition, the random selection of political representatives, is increasingly being used around the world to choose participants of deliberative processes like Citizens' Assemblies. Motivated by sortition's practical importance, there has been a recent flurry of research on sortition algorithms, whose task it is to select a panel from among a pool of volunteers. This panel must satisfy quotas enforcing representation of key population subgroups. Past work has contributed an algorithmic approach for fulfilling this task while ensuring that volunteers' chances of selection are maximally equal, as measured by any convex equality objective. The question, then, is: which equality objective is the right one? Past work has mainly studied the objectives Minimax and Leximin, which respectively minimize the maximum and maximize the minimum chance of selection given to any volunteer. Recent work showed that both of these objectives have key weaknesses: Minimax is highly robust to manipulation but is arbitrarily unfair; oppositely, Leximin is highly fair but arbitrarily manipulable. In light of this gap, we propose a new equality objective, Goldilocks, that aims to achieve these ideals simultaneously by ensuring that no volunteer receives too little or too much chance of selection. We theoretically bound the extent to which Goldilocks achieves these ideals, finding that in an important sense, Goldilocks recovers among the best available solutions in a given instance. We then extend our bounds to the case where the output of Goldilocks is transformed to achieve a third goal, Transparency. Our empirical analysis of Goldilocks in real data is even more promising: we find that this objective achieves nearly instance-optimal minimum and maximum selection probabilities simultaneously in most real instances -- an outcome not even guaranteed to be possible for any algorithm.

==> random-stuff.tex <==
\section{Linear straw man weaker results}
Unfortunately, this objective does not serve our goals. Formally, we can prove that there is no setting of $\gamma$ for which this objective is guaranteed to achieve $\Theta(1/n)$ selection probabilities for all agents, even if such a solution exists. First, we prove this for $\gamma = 1$ to get intuition \textcolor{orange}{(This toy case will ultimately be removed from the paper, it's just a stepping stone)}:

    
   \begin{theorem} There exists an instance in which there is a feasible solution of $[1/n\sqrt{n},\sqrt{n}/n]$, but:
   \begin{itemize}
       \item If $\gamma \leq n$, then the optimizer will give someone probability $O(1/n^2)$.
       \item If $\gamma > n$, the optimizer will give someone probability 1.
   \end{itemize}    
   
   
%       If $\gamma \in O(n)$ and there exists an instance with a feasible solution giving all people probabilities in $[1/n\sqrt{\gamma},\sqrt{\gamma}/n]$, the objective has an optimizer that gives someone probability $O(1/n^2)$. $O(1/(\gamma n))$.
        
       %If $\gamma \in \Omega(n)$, there exists an instance with a feasible solution giving all people probabilities in $[1/n\sqrt{n},\sqrt{n}/n]$, but the objective has an optimizer that gives someone probability 1.
   \end{theorem}
    \begin{proof}
        Use ideas above to prove --- first bound for $\gamma \in O(n)$ is in extension of the example in proposition 2 (``Extending this instance to larger $\gamma$), and the second bound for $\gamma \in \Omega(n)$ is in the proof of Proposition 3.

       \textbf{Case 1:} $\gamma\leq n$.

    Define the instance so that $n/4$ people have 00, $n/4$ people have 11, $1$ person as $01$, and $n/2$ people have $10$. We need perfect balance on both features.

   We know that $\nu_{01}/\nu_{10} = n/2$. Then, we have to decide where to position this requisite gap. If we position so that $\nu_{01}$ is order $\delta k/n$ with $\delta \in \omega(1)$ our objective is
   \[\delta k/n - \delta \gamma k / n^2 = \delta k/n (1 - \gamma/n).\]
    This nonnegative because $\gamma/n \leq 1$, so is clearly minimized when $\delta$ is as small as possible, so 1, in which case the minimum probability is $O(1/n^2).$
    
       
       %Construct the following instance: 1 person with 01, and $\gamma/2$ people with 10. and the rest of the people are split evenly between 00 and 11. Suppose we have that $p_{0,\cdot} = k/2$ and $p_{\cdot,0} = k/2$\emdash that is, we need 1/2 of the panel to have 0s in the first position, and 1/2 to have 0s in the second position. Then, we know that $\nu_{01} = \gamma/2 \cdot \nu_{10}$.

       %Suppose we give $n_{01}$ probability order $k/n$, and everyone in $00$ and $11$ order $k/n$. Then, 

        %$\nu_{10} = 2/\gamma \cdot \nu_{01} = 2/\gamma \cdot k/n$. Our objective value is
        %\[O(k/n) - \gamma \cdot 2/\gamma \cdot k/n \in O(k/n).\]

        %Say we give more probability to our group with 01, say $\delta k/n$ where $\delta \in \omega(1)$. Then, we give the $10$ people $2\delta k/n \cdot 1/\gamma$. Then, we get the difference
       %\[\delta k/n - 2 \gamma \delta k/n \cdot 1/\gamma  = \delta k/n \in \Omega(\delta k/n).\]

      % Therefore, to minimize the difference, we give no one more than $k/n$, meaning the worst-off people get $O(1/(\gamma n))$ \textcolor{red}{Can we drive this all the way down to $n^2$ for any $\gamma \leq n$?}
       

         \textbf{Case 2:} $\gamma(n) > n$.
         Use the same instance as above.  In this instance, We know $d^{dev} = n$, and the feasible solution we need exists. Now, we can assess the possible solutions' objective values. First, the balanced solution:
        \[\frac{\sqrt{n}}{n} - \gamma(n) \cdot \frac{1}{n\sqrt{n}} = \frac{1}{\sqrt{n}}\left( 1 - \frac{\gamma(n)}{n}\right)\]
        If we drive $i^*$'s probability  up 1, we get
        \[1 -  \frac{\gamma(n)}{n}.\]
%
        If $\gamma(n) > n$, both of these are negative and the second one is decreasing way faster, meaning that we will be incentivized to drive the maximum probability up to 1. 
    \end{proof}


    \textcolor{orange}{\textbf{Stronger case 1:}} $1 \leq \gamma\leq n$. There actually exists an instance in which the optimal solution is gives probabilities $[1/n\sqrt{\gamma},\sqrt{\gamma}/n]$ (so an even friendlier instance) but our objective gives someone $O(1/n^2)$.

    Define the instance so that $n/4$ people have 00, $n/4$ people have 11, $1$ person as $01$, and $\gamma/2$ people have $10$. We need perfect balance on both features.

     We know that $\nu_{01}/\nu_{10} = \gamma^{1+\epsilon}/2$. Then, we have to decide where to position this requisite gap. If we position so that $\nu_{01}$ is order $\delta k/n$ with $\delta \in \omega(1)$ our objective is
    \[\delta k/n - \delta \gamma k / (n\gamma^{1+\epsilon}) = \delta k/n (1 - \gamma/\gamma^{1+\epsilon}).\]
    This nonnegative because $\gamma/\gamma^{1+\epsilon} \leq 1$, so is clearly minimized when $\delta$ is as small as possible, so 1, in which case the minimum probability is $O(1/n^2).$
    


    \textcolor{orange}{\textbf{This does not capture the idea that, because the best possible gap can be $\Omega(k/n)$ due to \textit{constants}, we might actually give someone 0.}} 


    \begin{conjecture}
        for all $\gamma \leq n/3-1$, there exists an instance in which there exists a feasible solution that gives probabilities in $[\Omega(1/n\sqrt{\gamma}),O(\sqrt{\gamma}/n)]$, but the optimizer of \Cref{eq:obj_maxmin} gives an agent 0 probability by the above objective.
    \end{conjecture}
    \begin{proof}
        Let $3 k/4$ be the number of people we need with a vector of the form $(0,\cdot)$ and let $k/4$ be the number of people we need with a vector of the form $(\cdot,0)$. Let $n_{00} = n_{11} = n/6$, $ n_{01} = n/(3\gamma + 3)$, and $n_{10}$ be the rest.

        Now, we reduce the problem via the constraints (in mathematica), getting
    \[q_{01} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + 2\gamma) \qquad \text{and}\qquad q_{00} = q_{11} = \frac{3 k}{2 n} - q_{10} \frac{2 (1+ 2 \gamma)}{1 + \gamma}\]
    Now, it's clear that for all values of $q_{10} \in [0,1]$, we have that $q_{01} > q_{00}$, so the problem reduces to minimizing \[q_{01} - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + 2\gamma) - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + \gamma)\]
    This is minimized when $q_{10}=0.$
    \textcolor{red}{I think you can really crank on this instance and get the required upper bound on $\gamma$ arbitrarily close to $n$ from below}
    \end{proof}

    I now think the correct claim is roughly the following (but for the record, Theorem 3 is already enough to show separation between this objective and ours)

 \noindent \textbf{Case 1:} $\gamma \in [0,2]$. Fix an instance with two binary features, each with values in $\{0,1\}$. Suppose we need $3k/4$ 0s in the first position and $3k/4$ 1s in the second position. Now, suppose we have $n_{00} = n_{11} = n_{01} =n/6$; let $n_{10} = n/2$. 

       \noindent \textit{Establishing the existence of a good feasible solution:} %Assemble 1 type of panel: $k/12$ seats for 00, $k/12$ seats for 11, $2k/3$ seats for 01, and $k/6$ seats for 10. Observe that this satisfies the quotas: there are $k/12 + 2k/3 = 9k/12 = 3k/4$ 0s in the first position, and $k/12 + k/6 = k/4$ seats for 0s in the second feature. Define a panel distribution that randomizes uniformly over panels of this type; then the 
       Set the selection probabilities to $q_{10} = \nicefrac{k}{3n}, q_{01} = \nicefrac{4k}{n}, q_{00}=q_{11} = \nicefrac{k}{2n}.$ \textcolor{red}{By the reduction, we can realize this in a real instance for some $k,n$.}
    
       \noindent \textit{Computing the optimizer:} Now, we reduce the constraints using Mathematica to be in terms of $q_{01}$ and get that
       \[q_{01} = \frac{3k}{n} + 3q_{10} \qquad \text{and} \qquad q_{00} = q_{01} = \frac{3k}{2n} - 3q_{10}.\]
       By these expressions, we deduce that $q_{01}$ must be the largest probability, so our objective value is as follows, where the inequality uses that $\gamma \in [0,2]$:
       \[\max \left\{  \frac{3k}{n} + 3q_{10} - \gamma q_{10},  \frac{3k}{n} + 3q_{10}- \gamma \left(\frac{3k}{2n} - 3q_{10}\right)\right\} \geq \max\left\{\frac{3k}{n} + q_{10},3q_{10} \right\}\] 
       subject to the remaining constraints that all probabilities are in $[0,1]$. 
        For the entire domain of $q_{10}$, both of these functions are increasing in $q_{10}$; thus, this objective is minimized when $q_{10} = 0$. In the optimal solution, it must be the case that $q_{10} = 0$.\\
 %Let $3 k/4$ be the number of people we need with a vector of the form $(0,\cdot)$ and let $k/4$ be the number of people we need with a vector of the form $(\cdot,0)$. Let $n_{00} = n_{11} = n/6$, $ n_{01} = n/(3\gamma + 3)$, and $n_{10}$ be the rest.

%        Now, we reduce the problem via the constraints (in mathematica), getting
  %  \[q_{01} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + 2\gamma) \qquad \text{and}\qquad q_{00} = q_{11} = \frac{3 k}{2 n} - %q_{10} \frac{2 (1+ 2 \gamma)}{1 + \gamma}\]
  %  Now, it's clear that for all values of $q_{10} \in [0,1]$, we have that $q_{01} > q_{00}$, so the problem reduces to minimizing \[q_{01} - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + 2\gamma) - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + \gamma)\]
  %  This is minimized when $q_{10}=0.$

       \noindent \textbf{Case 2:} $2 < \gamma < n$. For this case, we design a slightly finer-tuned version of the above instance.
      Suppose we need the following numbers of 0s in the first and second positions, respectively:
       \[k/2\left(1 - \frac{1}{1 - \gamma(1 - 2 \epsilon)}\right)\quad \text{and} \quad k/2 \left(1 + \frac{1}{1 - \gamma(1- 2 \epsilon)}\right)\]
    Now, define the pool fractions as 
    \[\nu_{00} = \nu_{11} = \frac{1}{2} - \frac{1}{\gamma} - \epsilon, \quad \nu_{01} = 1/\gamma\]
    and $\nu_{10}$ is the rest. We set $\epsilon$ small enough so that all of these quantities are positive.

  \noindent \textit{Establishing the existence of a good feasible solution:}     
    \textcolor{red}{This instance has a solution that gives everyone in $[1/(\gamma n), \gamma/n]$}

    \noindent \textit{Computing the optimizer:}
    Reducing the constraints in Mathematica, we get that 
    \[q_{01} = \frac{ \gamma k/n}{\gamma(1-2\epsilon)-1} +  2\gamma \epsilon \cdot q_{10} \qquad \text{and} \quad q_{00}= q_{11} = \frac{\gamma k/n}{\gamma(1-2\epsilon)-1} - \frac{1 + 2 \epsilon}{\gamma (1 - 2 \epsilon) - 2} \cdot q_{10}.\]
    By these expressions, we deduce that $q_{01}$ must be the largest probability, so our objective value is as follows:
    \[\max\left\{ \frac{ \gamma k/n}{\gamma(1-2\epsilon)-1} +  2\gamma \epsilon \cdot q_{10} - \gamma q_{10}\right\}\]
    \textcolor{red}{$q_{10}$ is the smallest probability, and the box constraints don't bind.}
    For all values of $q_{10}$, $q_{01}$ dominates $q_{00}$ and $q_{11}$; therefore, minimizing the difference means minimizing $q_{01} - q_{10}$. This is minimized when $q_{10}=0$, given the positive coefficient on $q_{10}$.

        \textbf{Case 2.5:} $\gamma \leq n/3-1$. Let $n \geq 3k$
        
        Let $k/2 + (n3-1-\gamma)*k/4$ be the number of people we need with a vector of the form $(0,\cdot)$ and let $k/2 - (n3-1-\gamma)*k/4$ be the number of people we need with a vector of the form $(\cdot,0)$. Let $n_{00} = n_{11} = n/6$, $ n_{01} = n/(3\gamma + 3)$, and $n_{10}$ be the rest.
        
        \textit{Computing the optimizer.} Now, we reduce the problem via the constraints (in mathematica), getting
        \[q_{01} = \frac{k(\gamma+1)(n-3(\gamma+1))}{n(n-6)} + q_{10}(2\gamma + 1) \qquad \text{and} \qquad q_{00} = q_{11} = \frac{k(2n+3\gamma-15)}{n(n-6)} - q_{10}\frac{2(2\gamma + 1)}{\gamma+1}\]
        Plus the remaining box constraints. Handling the box constraints:
        \begin{itemize}
            \item For $q_{01}$, we clearly have that $q_{01} \geq 0$ for the entire range of $q_{10}$. In order to make sure $q_{01} \leq 1$, we need that 
            \[\frac{k(\gamma+1)(n-3(\gamma+1)}{n(n-6)} +  q_{10}(2\gamma + 1) \leq 1\iff q_{10} \leq  \frac{1}{1+2\gamma} - \frac{k(\gamma+1)(n-3(\gamma+1))}{n(n-6)(1+2\gamma)}\]
            To show that the right hand side is nonnegative for all $\gamma \in [1, n/3-1]$, it is sufficient to show that 
            \begin{align*}
                \frac{1}{1+2\gamma} - \frac{k(n-3(\gamma+1))}{n(n-6)} \geq 0 \iff 1 - \frac{k(n-3(\gamma+1))(1+2\gamma)}{n(n-6)} \geq 0
            \end{align*}
            This is quadratic in $\gamma$ with a positive leading coefficient, which means it's convex in $\gamma$. We take the derivative and set it equal to 0 (mathematica), 
            \item For $q_{00}, q_{11}$, we see that for all 
        \end{itemize}

        By inspection, we see that for all $q_{10} \in [0,1]$, it holds that $q_{01} > q_{00}$ and $q_{01} > q_{10}$. Therefore, $q_{01}$ is the maximum. 
        
        
        so the problem reduces to minimizing \[q_{01} - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + 2\gamma) - \gamma q_{10} = \frac{3 (1 + \gamma) k}{2 n} + q_{10}(1 + \gamma)\]
    This is minimized when $q_{10}=0.$\\
        \textbf{Case 2.75:} 


\section{Old attempts for breaking the linear combination}
------------------------------ I actually think the following proposition is wrong  --------------------------------
    \begin{proposition} \label{prop:mixobj_gmin0}
        If $\gamma = 1$, then there exists an instance in which there is a feasible solution that gives all agents in $\Theta(1/n)$ probabilities, but $\min_{i \in [n]} \pi_i = 0$.
    \end{proposition}
    \begin{proof}\textit{(sketch)}
        \textcolor{red}{Formalize this:} Consider an instance where there are two binary features, and the pool is composed of $n/6$ with $00$, $n/6$ with $01$, $n/6$  with $11$, and $n/2$ with $10$. The quotas require that the panel contains $2k/3$ people with a 0 in the first position and $k/3$ people with a 0 in the second position.

        \textbf{Claim 1:} there exists a solution giving all agents $\Theta(k/n)$ probability. \textit{Proof:} Choose one panel composition deterministically: $k/6$ seats for $00$, $k/6$ seats for 11, $k/2$ seats for 01, and $k/6$ seats for 10. Then, probabilities are $q_{00} = q_{11} = k/n$, $q_{01} = 3k/n$, and $q_{10} = k/(3n)$. This satisfies the quotas and all agents get probabilities order $k/n$.
        
        In order for the quotas to be satisfied, you can deduce that $q_{01} \propto 6 q_{10}$, because the probability assigned to the group 01 must be 2x the probability assigned to group 10, and there are 3x fewer people. Moreover, $q_{01}$ must be the largest probability due to the skew of the quotas. If $q_{01}$ must grow at 6x time the rate of $q_{10}$, the difference $q_{01} - q_{10}$\emdash which amounts to the difference between the max and min probability overall (to prove)\emdash must be minimized when $q_{10} = 0$.

        \textcolor{blue}{we can extend this proof to any constant $\gamma$.}
        % You can really use any instance like this, so long as the $10$ group is strictly bigger than the other groups, and the quotas are skewed to make the $01$ group extra valuable. The more severe these trends are, the worse the instance gets.
    \end{proof}
    %The high-level intuition here is that we know the smallest the difference can be is $O(k/n)$ in the general case (where quotas any mandate gaps). However, because the average probability must also be $k/n$ (of the same order), sometimes this distance will be smallest when some people are given 0. 

    \textbf{Extending this instance to larger $\gamma$.} Now, suppose we have $n^{1-\ell}/6$ people with 01, $n/6$ people with 11, $n/6$ people with 00, and the rest (order $n$) are 10. Now, the probability given to people with 01 will be $2n^\ell$ (roughly) times that given to 10, because we need 2x the probability assigned to group 01 and there are $n^\ell$ times fewer people. If $\gamma < 2n^\ell$, then I think we will give those with 10 probability 0, for the same reasoning as above. 

    Of course, this will induce a necessary multiplicative gap in the selection probabilities of $n^{\ell}$, which means that as $\ell$ increases, the existing feasible instance gets worse. Doing some examples:

    If $\ell = 1$, then $\gamma < 2n$ will result in giving people with 10 probability 0, but there exists a solution that gives people probabilities in the range $[1/n\sqrt{n}, 1/\sqrt{n}]$.

    For general $\ell$, $\gamma < 2n^{\ell}$ will give someone probability 0, while the best instance we could find will give people probabilities in the range $[1/n\sqrt{n^{\ell}}, \sqrt{n^{\ell}}/n]$.
    
    We have proven a bad example up to the case where $\gamma $ is up to $O(n)$. We can't push this any further because otherwise we will have fractional people in vector group 01. 
    
    Now, we need a different approach to cover larger values of $\gamma$, which in which case the concern is that we \textit{overshoot} the max probability, as this objective will encourage us to do whatever it takes to increase the minimum probability. We can study the case where $\gamma(n) > \omega(n)$ below.

    \begin{proposition}
        If $\gamma(n) >n$, then in an instance where there is a feasible solution that gives $[1/n\sqrt{n}, \sqrt{n}/n$, but there also exists an optimizer that gives someone probability 1.
    \end{proposition}
    \begin{proof}
        Suppose that we use the instance from the lower bound below, where order $n$ agents report $01$, 1 agent $i^*$ reports 10, and everyone else is split evenly between 00 and 11. We need perfect balance. 

        In this instance, We know $d^{dev} = n$, and the feasible solution we need exists. Now, we can assess the possible solutions' objective values. First, the balanced solution:
        \[\frac{\sqrt{n}}{n} - \gamma(n) \cdot \frac{1}{n\sqrt{n}} = \frac{1}{\sqrt{n}}\left( 1 - \frac{\gamma(n)}{n}\right)\]
        If we drive $i^*$'s probability  up 1, we get
        \[1 -  \frac{\gamma(n)}{n}.\]
%
        If $\gamma(n) > n$, both of these are negative and the second one is decreasing way faster, meaning that we will be incentivized to drive the maximum probability up to 1. 
    
       % Note: We cannot use the same instance above to build such a case, because the maximum probability achievable in that instance is $1/n$. We therefore need to create a situation where order 1/n is possible, but giving someone 1 is preferable, \textit{while having a group be of constant size.} I don't know how to do this yet, but here is the intuition for what goes wrong:
    \end{proof}
   \begin{remark}
       I think we can also generalize this analysis to show that $\gamma(n) \in [\omega(1),o(n)]$ gives people too high of probability. However, what we can show is that if $\gamma(n)$ is in this range, then we can find an instance where there is a feasible solution with probabilities in $[1/n\sqrt{\gamma(n)}, \sqrt{\gamma(n)}/n]$ but we get a solution that gives someone probability $\gamma(n)/n$, which is a fair bit higher. As $\gamma(n) \to 1$, this becomes very weak, as we are doing little worse on the upper end than the best possible. 
   \end{remark} 

   \textcolor{orange}{\textbf{Synthesizing this into the proposed theorem, which works entirely with asymptotics:}}


\section{Lemma about combining lower bound instances}


    \textcolor{purple}{Sad news -- I think this lemma may only hold for objectives that are separable over $\pi_1, \dots, \pi_n$ and $\pi_{n+1}, \dots, \pi_{2n}$ (which would still hold for log barrier function if we use arbitrary p norm and not infinity norm). If we consider for example the max - min objective from above, consider combining a scenario where everyone can get exactly equal probability and one where the minimum possible max-min gap is achieved when max is $O(1/n)$ and min is $O(1/n^2)$. Then probabilities for the first subset of agents can kinda be whatever as long as they are in the leeway provided by the second instance. This case doesn't really matter if we care about min/max probabilities, but consider a more nefarious hypothetical case: we have an instance that gives us a min probability of 0 and an instance that gives us a max prob of 1, and assume that the objective value of the first instance is bigger than in the second. What if there exists some assignment of probabilities for the second instance such that the max-min gap on those agents is bigger but the max is less than 1? Then already we have an assignment of probs such that the overall objective value is less than what it was before, but it messes up our max prob instance. }
    
    Attempting to formalize our ability to do this by the following lemma. If I didn't make a mistake, the following lemma allows us to combine the two instances:
    \begin{lemma} \label{lem:combine-instances}
        Fix an arbitrary objective function $g$ and two instances (for simplicity, suppose $n$ and $k$ are the same across instances, and each instance has two binary features). We can construct a new instance in which \textit{all agents from both instances receive the same selection probabilities according to the objective $g$} as in their original respective instances.
    \end{lemma}
    \begin{proof}\textit{(sketch)}
        Call the instances $I, I'$. Create a new instance with all agents across both pools $N,N'$ (so the new pool is size $2n$), a panel of size $2k$. This instance will have 4 features.

        For each feature in instance $I$, for all $i \in N$, let $i$'s values for that feature (which are in 0,1) remain the same. For all $i \in N'$, set $i$'s value for this feature to \textit{2} (note that this feature is no longer binary). Keep the quotas on 0 and 1 the same, and additionally require that exactly $k$ agents with value 2 are chosen for the panel. 
        
        Repeat this process for instance $I'$. 

        Due to the quotas, we have to take exactly $k$ agents from instance 1 and $k$ agents from instance 2. We can therefore reduce the problem to the original two separate instances, and we have satisfied all quotas on value 2 of all features. Now, each individual sub-instance corresponds exactly to one of our two original instances $I,I'$.


     \textcolor{red}{If the $g$ objective in instance $I$ gives those agents $\pi^g$ and in instance $I'$ gives agents $\pi^g \, '$, then by the convexity of $g$, the global optimizer over all inputs in these two instances will give all agents the same probabilities as before.}

     \textcolor{purple}{To show it holds for separable objectives, I think you just need to argue that all marginals from the original problem can be realized in this variant while leaving the marginals from the other instance unchanged}
    \end{proof}



%    \textbf{\textcolor{red}{Can we prove these negative results are tight?}}


  %  \textcolor{red}{\textbf{Can we prove something about \textit{general} combinations of distributions?} Ideally, something like ``in the general case, combining distributions with any weight can never give you better than $X$.'' It would be great for the story if we could destroy this entire approach, since the current version leaves open the prospect of combining other distributions.}


    
    
    
    
%        Suppose we have an instance where there is some $i$ and $i'$ such that
%        \begin{enumerate}
%            \item $\pi_i^{\textsc{Minimax}} = \pi_{min}^{\textsc{Minimax}} = 0$
%            \item $\pi_i^{\textsc{Maximin}}  = \pi_{min}^{\textsc{Maximin}} \in \Theta(1/n)$ (trivial)
%            \item $\pi_{max}^{\textsc{Minimax}} \in \Theta(1/n)$ (trivial)
%            \item $\pi_{max}^{\textsc{Maximin}} \in \Omega(1)$. 
%        \end{enumerate}

        
 %       2 and 3, as noted above, are trivial as they are true in any instance: the \textsc{Minimax} solution has maximum probability in $O(1/n)$ as proven in the previous paper, and the \textsc{Maximin} solution gives everyone probability $\Omega(1/n)$ by the fact that we can always find a single panel per person and uniformly randomize over them, thereby giving everyone probability at least $1/n$ in the optimal solution.

  %      Finding an instance in which 1 and 4 and true simultaneously is the trick. First, we will show that such an instance is enough to prove the claim; then, we will find such an instance.

  %      If we have such an instance
   % \end{proof}

    
%    \subsection{Straw Man 2: Log barrier function} The problem with \Cref{eq:obj_maxmin} is that the $\min$ term is in some sense too ``weak'' --- the objective does not sufficiently strongly penalize low probabilities, because the objective increases only linearly as the minimum probability decreases. Flanigan \textit{et al} propose another objective, the infinity norm with a log barrier function, which is effectively a modification of \Cref{eq:obj_maxmin} which steepens the rate of increase in the objective as the minimum probability declines:
 %   \[\min_{\cal D} \  \max_{i \in [n]}\pi_i + \gamma\left(-\sum_{i \in [n]}\log(\pi_i)\right)\]
    
    
 %   We show that this can be no better than 

 %   \textcolor{red}{Try to find counterexample to show gap}

\section{Old Goldilocks}


   \begin{proposition}
        Fix $\boldsymbol{\pi}$ and let $\max :=\max_{i \in [n]}\pi_i$ and likewise, $\min :=\min_{i \in [n]}\pi_i$.
        \[\lim_{p \to \infty} \left(\sum_{i \in [n]}\pi_i^p\right)^{1/p} + \gamma \left(\sum_{i \in [n]} \frac{1}{\pi_i^p}\right)^{1/p} = \max + \gamma \frac{1}{\min}\]
    \end{proposition}
    \begin{proof}
        We'll analyze the two terms separately, both in much the same way:
        \begin{align*}
            \max = (\max \, ^p)^{1/p} \leq \left(\sum_{i \in [n]} \pi_i^p\right)^{1/p} \leq \left(\sum_{i \in [n]} \max\, ^p\right)^{1/p} = n^{1/p}  \max \xrightarrow[]{p \to \infty} \max
        \end{align*}
        \begin{align*}
            \frac{1}{\min} = \left(\frac{1}{\min \, ^p}\right)^{1/p} \leq \left(\sum_{i \in [n]} \frac{1}{\pi_i}^p\right)^{1/p} \leq \left(\sum_{i \in [n]} \frac{1}{\min\, ^p}\right)^{1/p} = n^{1/p} \frac{1}{\min} \xrightarrow[]{p \to \infty} \frac{1}{\min} \quad \qedhere
        \end{align*}
    \end{proof}
        %We're analyzing a slightly different objective, with both terms individually raised to the $p$, which is serving to more strongly penalize both high max and low min:
    %\[ \sum_{i \in [n]}\pi_i^p + \gamma \sum_{i \in [n]} \frac{1}{\pi_i^p} \]

    %While it's weird to understand the behavior of this as $p \to \infty$, we can understand the behavior of another, very similar objective where $z \in [1,p)$ is a constant:
%\[\lim_{p \to \infty} \left(\sum_{i \in [n]}\pi_i^p\right)^{z/p} + \frac{\gamma}{h(n,p,z)} \left(\sum_{i \in [n]} \frac{1}{\pi_i^p}\right)^{z/p} = \max \, ^z + \gamma \frac{1}{\min^z}\]

    
    \begin{theorem} \label{thm:goldilocks}
    Suppose there exists a feasible solution $\pi$ in which $\pi_i \in \left[\frac{1}{d(n) \cdot n}, \frac{d(n)'}{n}\right]$ for all $i \in [n]$, where $d(n), d'(n) \in \Omega(1)$. Then, let $\pi^*$ be the optimizer of the following objective in this instance:
\[f_{gold}(\pi) = \left(\sum_{i \in [n]}\pi_i^p\right)^{1/p} + \frac{1}{n^{2}}\left(\sum_{i \in [n]}\frac{1}{\pi_i^p}\right)^{1/p}.\]
Then, for all $i \in [n]$, we have that
\[\pi_{i}^* \in \left[\frac{1}{2 n^{1+1/p}} \cdot \frac{1}{\max\{d(n), d'(n)\}}, \ \frac{2}{n^{1-1/p}} \cdot \max\{d(n), d'(n)\} \right].\]
\end{theorem}
\begin{proof}
First, we start with our feasible solution and upper bound the objective:
\begin{align*}
f_{gold}(\pi) = \left(\sum_{i \in [n]}\pi_i^p\right)^{1/p} + \frac{1}{n^{2}}\left(\sum_{i \in [n]}\frac{1}{\pi_i^p}\right)^{1/p} 
%
&\leq \left(\sum_{i \in [n]}\left(\frac{d(n)'}{n}\right)^p\right)^{1/p} + 
\frac{1}{n^{2}}\left(\sum_{i \in [n]}\left(\frac{1}{d(n) \cdot n}\right)^p\right)^{1/p}\\
%
&= \frac{d'(n)}{n^{1-1/p}} + \frac{d(n)}{n^{1-1/p}}\\
%
&\leq \frac{2}{n^{1-1/p}}\max\left\{d(n),d'(n)\right\}
\end{align*}

Now, assume for the sake of contradiction that in the optimizer $\pi^*$, someone receives higher-order probability than $\frac{2}{n^{1-1/p}} \cdot \max\{d(n), d'(n)\}$. Then, 
\begin{align*}
f_{gold}(\pi^*) > \frac{2}{n^{1-1/p}} \cdot \max\{d(n), d'(n)\} 
\end{align*} 
which is a contradiction to the optimality of this solution. Likewise, assume for the sake of contradiction that in the optimizer $\pi^*$, someone receives lower-order probability than $\frac{1}{2 n^{1+1/p}} \cdot \frac{1}{\max\{d(n), d'(n)\}}$. Then,
\begin{align*}
f_{gold}(\pi^*) > \frac{2 n^{1+1/p} \cdot \max\{d(n), d'(n)\}}{n^{2}} 
& = \frac{2}{n^{1 - n^{1-1/p}}}\cdot \max\{d(n), d'(n)\}
\end{align*}
Again, encountering a contradiction. We conclude the claim.
\end{proof}

%From this result, we can see that what matters to the performance of this objective is the existence of a feasible solution with a small multiplicative gap between minimum and maximum probabilities. For a given instance $I$, define $\phi(I)$ to be the smallest multiplicative gap in selection probabilities that exists in any feasible solution in instance $I$.
% Observe that for a fixed gap size $\phi$, our algorithm performs best if this gap is positioned \textit{symmetrically} around $1/n$; that is, where the probabilities are bounded between $[\nicefrac{1}{\sqrt{\phi} n}, \nicefrac{\sqrt{\phi}}{n}]$. 
    
%    \begin{observation}[The benefit of \textit{symmetric} deviation] \label{obs:symm}
 
 %   \end{observation}
    

\section{Older Goldilocks}
\begin{theorem} \label{thm:goldilocks}
    Suppose there exists a feasible solution $\pi$ in which $\pi_i \in [1/n^{m}, 1/n^{q}]$ for all $i \in [n]$, where $m \geq 1 \geq q$. Then, let $\pi^*$ be the optimizer of the following objective in this instance, where $z \in (0, p]$ is a constant:
\[f_{gold}(\pi) = \left(\sum_{i \in [n]}\pi_i^p\right)^{1/p} + \frac{1}{n^{2}}\left(\sum_{i \in [n]}\frac{1}{\pi_i^p}\right)^{1/p}.\]
Then, for all $i \in [n]$, we have that
\[\pi_{i}^* \in \left[\frac{2}{n^{\max\{m+1/p, 2-q+1/p\}}},\frac{1/2}{n^{\min\{q-1/p, 2-m-1/p\}}}\right].\]
\end{theorem}
\begin{proof}
First, we start with our feasible solution and upper bound the objective:
\begin{align*}
f_{gold}(\pi) = \left(\sum_{i \in [n]}\pi_i^p\right)^{1/p} + \frac{1}{n^{2}}\left(\sum_{i \in [n]}\frac{1}{\pi_i^p}\right)^{1/p} 
&\leq \left(\sum_{i \in [n]}\left(\frac{1}{n^q}\right)^p\right)^{1/p} + \frac{1}{n^{2}}\left(\sum_{i \in [n]}(n^{m})^p\right)^{1/p}\\
&= \frac{1}{n^{q-1/p}} + \frac{1}{n^{2-m-1/p}}\\
&\leq \max\left\{\frac{2}{n^{q-1/p}},\frac{2}{n^{2-m-1/p}}\right\}\\
&= \frac{2}{n^{\min\{q-1/p,2-m-1/p\}}}
\end{align*}

Now, assume for the sake of contradiction that in the optimizer $\pi^*$, someone receives higher-order probability than $\frac{2}{n^{\min\{q-1/p, 2-m-1/p\}}}$. Then, 
\begin{align*}
f_{gold}(\pi^*) > \frac{2}{n^{\min\{q-1/p, 2-m-1/p\}}} = \frac{2}{n^{ \min\{q-1/p, 2-m-1/p\}}}
\end{align*} 
which is a contradiction to the optimality of this solution. Likewise, assume for the sake of contradiction that in the optimizer $\pi^*$, someone receives lower-order probability than $\frac{1}{2n^{\max\{m+1/p, 2-q+1/p\}}}$. Then,
\begin{align*}
f_{gold}(\pi^*) > \frac{2n^{\max\{m+1/p, 2-q+1/p\}}}{n^{2}} 
&= \frac{2}{n^{2 - \max\{m+1/p, 2-q+1/p\}}}\\
&= \frac{2}{n^{\min\{2- (m+1/p), 2 - 2+q-1/p)\}}}\\
&= \frac{2}{n^{\min\{2-m-1/p, q-1/p)\}}}
\end{align*}
Again, encountering a contradiction. we conclude the claim.
\end{proof}
 
 
 \section{Combined \textit{panel distributions} for max/min}
    \textcolor{blue}{We should be able to prove that this is always weakly worse than the multi-objective}
    Another way to combine the goals of \textsc{Maximin} and \textsc{Minimax} would be to to average the \textit{panel distributions} that each of these objectives produces individually. We can show that there is no weighted average of these distributions guaranteed to give $\Theta(1/n)$. We define this generic weighted average as
    \[\mathcal{D}:= \frac{\mathcal{D}^{\textsc{Maximin}} +  \gamma(n) \mathcal{D}^{\textsc{Minimax}}}{1 + \gamma(n)}.\] 

    First, clearly, if $\gamma(n)$ is constant, we're giving equal weight to both distributions and we're screwed: if the \textsc{Maximin} optimal gives someone probability 1, then the max probability in the average will be constant.
    The only reasonable option, then, is to start increasing $\gamma$ in order to to more heavily weight the $\textsc{Minimax}$ distribution in the average. However, perhaps unsurprisingly, we exchange this benefit to the maximum probability for a loss in the minimum probability:
    \begin{theorem}
        If $\gamma(n) \in \omega(1)$, then the minimum probability can be as low as
        \[O\left(\frac{1}{n\gamma(n)}\right).\]
    \end{theorem}
    \begin{proof}\textit{(Sketch)}
    Suppose we have an instance where there is some $i$ such that it gets (order of) the minimum amount of probability by both \textsc{Minimax} and \textsc{Maximin}:
    \[\pi_i^{\textsc{Minimax}} = \pi_{min}^{\textsc{Minimax}} = 0\]
    and
    \[\pi_i^{\textsc{Maximin}}  = \pi_{min}^{\textsc{Maximin}} \in \Theta(1/n).\]
    \textcolor{blue}{I believe we have an instance like this: The instance used to prove \Cref{prop:mixobj_gmin0}.
  }

    In such an instance, in the average of the two distributions, $i$'s selection probability is
    \[\frac{\Theta(1/n) + 0}{1 + \gamma(n)} \in O\left(\frac{1}{n\gamma(n)}\right),\]
    as needed.
      \end{proof}
    As $\gamma(n) \to \Theta(1)$, the less severe this lower bound gets. We now formalize the tradeoff that as $\gamma(n) \to \Theta(1)$, the worst-case maximum probability grows higher:
    \begin{theorem}
        If $\gamma(n) \in \omega(1)$, then the maximum probability can be at least
        \[\pi^*_{\max} \in \Omega\left(\frac{1}{\gamma(n)}\right)\] 
    \end{theorem}
    \begin{proof} \textit{(Sketch)}
    Suppose we have an instance where there is some $i$ such that it gets (order of) the maximum amount of probability by both \textsc{Minimax} and \textsc{Maximin}:
    \[\pi_i^{\textsc{Minimax}} = \pi_{\max}^{\textsc{Minimax}} = \Omega(1/n)\]
    and
    \[\pi_i^{\textsc{Maximin}}  = \pi_{\max}^{\textsc{Maximin}} \in \Omega(1).\]
    \textcolor{blue}{I believe we do have such an instance; the instance used to prove the lower bound on maximin in the original manipulation paper.}
    
    Then, the objective will give $i$ selection probability
    \[\frac{1 + \gamma(n) \Omega(1/n)}{1 + \gamma(n)} \in \Omega\left(\frac{1}{\gamma(n)} + \frac{1}{n}\right) \in \Omega\left(\frac{1}{\gamma(n)}\right). \qedhere\]
    \end{proof}

    \textcolor{blue}{\textbf{Note:} One weakness of these two negative results is that one could argue that, because we compute the distributions \textit{before} combining them in some weighted way, you could choose $\gamma(n)$ in an instance-dependent way \textit{after seeing the distributions}. What we really need to destroy this claim is a single instance in which both of these negative results hold simultaneously. I think we might be able to do this by combining the two instances into a 4-feature instance.}





     %\begin{theorem}
    %    If there \textbf{exists} some (unknown) panel distribution that gives all agents in $\left[\frac{c_1}{n}, \frac{c_2}{n}\right]$ selection probabilities, then the \textsc{FF}-optimal selection probabilities $\pi^{\textsc{FF}}$ satisfies that 
    %    \[\pi^{\textsc{FF}}_i \in \left[\Omega\left(\frac{1}{n^{1+1/p}}\right), O\left(\frac{1}{n^{1-2/p}}\right)\right] \quad \text{for all } i \in [n]\]
    %\end{theorem}
    %To prove this, we first prove something more general:
    %\begin{lemma}
    %    Fix any $m,q$ such that $m \geq 1 \geq q$ and $\frac{1}{2 - m - q} = p$. Then, if there exists a panel distribution $\mathcal{D}$ with corresponding $\pi$ whose corresponding marginals in $\pi$ are in $[1/c_1n^m,c_2/n^q]$ for all agents
        %We begin by showing that if we have a feasible solution, $\mathbf{\pi}$, that gives all agents at most $O(\frac{1}{n^q})$ probability and at least $\Omega(\frac{1}{n^m})$ probability for some $m \geq 1 \geq q$ such that $qp = 2p-mp-1$, 
   %     then the optimal panel distribution $\mathcal{D}^{FF(p)}$ will assign all agents selection probabilities in the range within 
   %     \[\left[\frac{c_1}{n^{m+1/p}},\frac{c_2}{n^{q-1/p}}\right]\]
   % \end{lemma}
   % \begin{proof}
   %       Our approach will be to upper-bound $\textsc{FF}(\pi)$, and then argue that having any agents probabilities in $\pi^{FF(p)}$ outside the desired bounds will imply that $\textsc{FF}(\pi^*)$ is worse than this upper bound. 
          
    %      \textbf{Upper bound on $FF^p(\pi)$.} We can upper bound $\textsc{FF}(\pi)$ by individually bounding each of the terms:\begin{align*}
    %        \textsc{FF}^p(\mathbf{\pi}) = \|\mathbf{\pi}\|_p^p + \gamma\frac{1}{n^{2p-1}} \sum_{i \in [n]} \frac{1}{\pi_i^p}
     %       &\leq \sum_{i \in [n]} \left(\frac{c_2}{n^q}\right)^p + \gamma c_1^p\sum_{i \in [n]} \frac{n^{mp}}{n^{2p-1}}\\
    %        &=c_2^p \cdot \frac{1}{n^{qp-1}} + \gamma c_1^p \cdot \frac{1}{n^{2p-mp-2}}\\
            %&= O\left(n \cdot \frac{1}{n^{qp}}\right) + O\left(n \cdot \frac{n^{mp}}{n^{2p-1}}\right)\\
            %&= O\left(\frac{1}{n^{qp-1}}\right) + O\left(\frac{1}{n^{2p-mp-2}}\right)\\
    %        \intertext{By assumption on $m$ and $q$, we have that $p = 1/(2-m-q) \iff 2p- mp - 2 = qp-1$, meaning that }
    %        &= \left(c_2^p + \gamma c_1^p \right) \cdot \frac{1}{n^{qp-1}}
    %    \end{align*}
    %    \textcolor{red}{need to fix, weird stuff happening with constants $\gamma, c_1, c_2$. Have not yet integrated $z$.}

  %      \textcolor{blue}{My sense is that we can prove something more general about how close we can get to the best existent solution, but need to figure out how to write the statement.}
        
   %     \textbf{Upper bound on $\pi^{FF^p}$.} Now, we will prove that all entries of $\pi^{FF^p}$ are upper bounded by $(c_1 + c_2)/n^{q - 1/p}$. Assume for the sake of contradiction that there exists some agent $i$ such that $\pi^*_i > (c_1 + c_2)/n^{q - 1/p}$. By just considering the first term of $\textsc{FF}(\mathbf{\pi^*})$, we know that $\textsc{FF}(\mathbf{\pi^*}) \geq (\pi_i)^p$. implying that $\textsc{FF}(\mathbf{\pi^*}) > \left((c_1 + c_2)/n^{q - 1/p}\right)^p = (c_1 + c_2)^p \frac{1}{n^{qp - 1}} $. However, then we have that $\textsc{FF}(\mathbf{\pi^*})$ is asymptotically bigger then $\textsc{FF}(\mathbf{\pi})$, contradicting the optimality of $\pi^*$ \textcolor{purple}{is it an issue that this is asymptotic}. Therefore, for all $i$, we must have that $\pi^*_i \in O(\frac{1}{n^{q-1/p}})$.\\

        %To show the lower bound on the minimum probability in $\pi^*$, we similarly assume for sake of contradiction that there exists some agent $i$ such that $\pi^*_i \in o(\frac{1}{n^{m+1/p}})$. Then by looking only at the second term of the objective function, we know that $\textsc{FF}(\mathbf{\pi^*}) \geq \frac{1}{n^{2p-1}} \cdot \frac{1}{o(1/n^{mp + 1})} \in \omega(\frac{1}{n^{2p-mp-2}}) = \omega(\frac{1}{n^{qp-1}})$. This again contradicts the optimality of $\pi^*$. Hence, we have shown that for all $i$ we must have that  $\pi^*_i \in \Omega(\frac{1}{n^{m+1/p}})$ and $ \pi_i^* \in O(\frac{1}{n^{q-1/p}})$.
    %\end{proof}
    %    The proof proceeds in a few claims.

    %    \textbf{Claim 1.} S
        
        %$\mathbf{\pi^*}$ will assign all agents at most $O(\frac{1}{n^{q-1/p}})$ and at least $\Omega(\frac{1}{n^{m+1/p}})$ probability. 

  %      Now we can utilize our assumption that there exists a panel distribution $\mathcal{D}$ such that all of the marginals $\pi^{\mathcal{D}}_i \in \Theta(1/n)$ in conjunction with this more general framework. As $\pi^{\mathcal{D}}_i \in \Theta(1/n)$ for all $i$, we can more weakly say that $\pi^{\mathcal{D}}_i \in \Omega(\frac{1}{n})$ and $\pi^{\mathcal{D}}_i \in O(\frac{1}{n^{1-1/p}})$. So let $q = 1-1/p$ and $m = 1$. Note that indeed $qp = p - 1 = 2p - p -1 = 2p-mp-1$ as required. Then we have that $\pi^*$ assigns all agents at most $O(\frac{1}{n^{1-2/p}})$ probability and at least $\Omega(\frac{1}{n^{1+1/p}})$ probability, as claimed.
    %\end{proof}

    

    
    %will need to assume that there \textit{exists} a feasible solt
    %About our instance $N,k,FV,\boldsymbol{\ell},\boldsymbol{u}$ with corresponding $\mathcal{K}$, we assume the following:
%    \begin{assumption}[Minimal Feasibility]
  %      For all agents $i \in N$, there exists some $K \in \mathcal{K}$ such that $i \in K$.
 %   \end{assumption}
  %  \begin{assumption}[Pool Richness]
  %  $N$ contains some set of feature-vectors $\mathcal{W}^* \subseteq \mathcal{W}$ such that
   %     \begin{itemize} 
   %         \item[--] There is a constant $\kappa^*>0$ such that $\nu_w(N) \geq \kappa^* + k/n$ for all $w \in \mathcal{W^*}$, and
    %        \item[--] There exists a set of panels $\mathcal{K}^* \subseteq \mathcal{K}$ such that for all $K \in \mathcal{K}^*$, $K$ contains only agents $i : w(i) \in \mathcal{W}^*$. 
    %    \end{itemize}
    %\end{assumption}
    %\begin{claim}
     %   Together, these assumptions imply that there exists a panel distribution $\mathcal{D}$ whose corresponding marginals $\boldsymbol{\pi}^{\mathcal{D}}$ are such that for all $i$, $\pi_i^{\mathcal{D}} \in \Theta(1/n)$. 
    %\end{claim}
    %\begin{proof}
    %    The high-level intuition is that
   %     We will construct this distribution $\mathcal{D}$. First, consider the distribution $\tilde{\mathcal{D}}$, which randomizes uniformly over the panels in $\mathcal{K}$. For all vectors already receiving at least $2/|FV|$ total probability from this randomization, leave agents with these vectors alone. Let $\tilde{N}$ be the set of agents who have not received probability at least $1/n$ from this process. Now, for each $i \in \tilde{N}$, do the following procedure:
   %     \begin{itemize}
            \item find a panel they're on and add probability $1/(2n)$.
            \item remove all agents from set $i \in {\tilde{N}}$
        \end{itemize}  For every vector not receiving constant total probability (of which there can be at most constant, since $|FV|$ is constant in $n$), for each $i$ with that vector, add probability $1/(|FV|n)$ to a panel containing that individual, subtracting it equally from the probability allocated to each panel in $\mathcal{K}$. At each such step, check if other 

        No panel can get more than probability 1, so every agent with a vector $w \in \mathcal{W}$ has probability at most $O(1/n)$. No agent can get probability $1/n$, 
        
        If there were $x$ many such vectors, then the total probability given to 

        
        Let $\tilde{N}_1 \subseteq N$ be the set of vectors not included in least a constant fraction of the panels in $\mathcal{K}^*$, and let $\tilde{N}_2$ be the rest of the agents in $N$.

        Define $\mathcal{D}$ to place probability $1/2$ uniformly randomly over the panels in $\mathcal{K}$. Now for every $i \in \tilde{N}_1$, find a panel (can be or not be in the support of $\mathcal{K}$) in which $\tilde{i}$ is included (there must be at least one, by assumption 1); call this panel $K_{\tilde{i}}$. Add probability $1/(2|\tilde{N}$
        
        $\mathcal{\kappa^*}$. begin from the distribution that randomizes uniformly over the panels in $\mathcal{K}^*$. Let $\tilde{N} \subseteq $ be the set of agents $\tilde{i}$ who receive 0 probability from this randomization. Now, for every agent $\tilde{i}$ receiving 0 probability in this randomization $\mathcal{D}$, Take probability $1/(2n)$ away from the 

        Each vector group $w \in \mathcal{W}^*$ can receive total probability $1$ in this randomization and there are at least $\kappa^* n + k$ people of each vector in the pool, meaning that this randomization grants everyone maximum probability $1/(\kappa^* n + k) \in O(1/n)$ probability. 
    \end{proof}
